Logic-LM: Empowering Large Language Models with Symbolic Solvers for Faithful Logical Reasoning

Large Language Models (LLMs) have shown human-like reasoning abilities but still struggle with complex logical problems. This paper introduces a novel framework, Logic-LM, which integrates LLMs with symbolic solvers to improve logical problem-solving. Our method first utilizes LLMs to translate a natural language problem into a symbolic formulation. Afterward, a deterministic symbolic solver performs inference on the formulated problem. We also introduce a self-refinement module, which utilizes the symbolic solver's error messages to revise symbolic formalizations. We demonstrate Logic-LM's effectiveness on five logical reasoning datasets: ProofWriter, PrOntoQA, FOLIO, LogicalDeduction, and AR-LSAT. On average, Logic-LM achieves a significant performance boost of 39.2% over using LLM alone with standard prompting and 18.4% over LLM with chain-of-thought prompting. Our findings suggest that Logic-LM, by combining LLMs with symbolic logic, offers a promising avenue for faithful logical reasoning. Code and data are publicly available at https://github.com/teacherpeterpan/Logic-LLM.

==> backup.tex <==
% 1. LLM has strong logical reasoning ability. 

% Logical reasoning is essential to human cognition and intelligence, enabling us to draw conclusions, make predictions, and solve problems based on given information. 
Logical reasoning is a cognitive process that involves using evidence, arguments, and logic to arrive at conclusions or make judgments~\cite{DBLP:journals/corr/abs-2212-10403}. It plays a central role in intelligent systems for problem-solving, decision-making, and critical thinking. Recently, Large Language Models (LLMs)~\cite{DBLP:journals/corr/abs-2303-08774} have exhibited emergent ability to ``reason'' like human~\cite{DBLP:journals/corr/abs-2206-07682}. When prompted with step-wise explanations of reasoning (``chain of thoughts''), or a simple prompt ``Let’s think step by step.'', these models are able to answer questions with explicit reasoning steps~\cite{chaing_of_thought,DBLP:journals/corr/abs-2205-11916}. 

% 2. LLM is not designed for faithful reasoning. 
Despite the advances of LLMs, they still face challenges when it comes to complex logical reasoning problems [CITE]. Chain-of-thought may mimic human reasoning processes, but it does not guarantee the \textit{faithfulness of reasoning}, \textit{i.e.}, whether the generated explanation accurately represents the correct reasoning process. The unfaithfulness is arguably due to the fundamental nature of LLMs as probabilistic models that predict the next token. [CITE] In contrast, symbolic expert systems [CITE], are considered to be faithful because the reasoning is based on symbolic-represented knowledge and follows explicit inference rules that adhere to logical principles. 


% The fundamental nature of LLMs as probabilistic models that predict the next token makes them less reliable than symbolic inference engines where the reasoning is based on symbolic-represented knowledge and follows explicit inference rules that adhere to logical principles. 

% Despite the advances of LLMs, they still face challenges when it comes to complex logical reasoning problems. Prior works [CITE] revealed that LLMs occasionally generate unfaithful explanations that fail to accurately represent the correct reasoning process. Although chain-of-thought may mimic human reasoning processes, the fundamental nature of LLMs as probabilistic models predicting the next most probable token makes them less reliable and robust than deterministic symbolic solvers, which base the reasoning on symbolic-represented knowledge and follow explicit inference rules that adhere to logical principles. For example, given the premises ``All humans are mortal.'' and ``Socrates is human.'', a first-order logic (FOL) inference engine applies the Modus Ponendo rule on their FOL formulas $\forall x Human(x) \rightarrow Mortal(x)$ and $Human(Socrates)$ to derive the conclusion $Mortal(Socrates)$ (``Socrates is a mortal.''), which guarantees faithfulness. 


Related Works 

% different with previous neuro-symbolic methods that xxx (complex optimization), we propose a more succinct framework that fully utilizes the language understanding ability of LLMs to formulate the problem and then select the appropriate symbolic solver to help with the 
% compared with symbolic; we still center LLMs which is more generalizable. however, we adpot symbolic solvers as external modules to assist the reasoning which addresses the shortcoming of pure LLMs 


% Symbolic System
% The past research of logical reasoning within AI uses formal language (e.g., first-order logic) as knowledge representation and symbolic reasoners (Muggleton and Raedt, 1994). This paradigm has resulted in impressive applications such as expert systems (Metaxiotis et al., 2002).

% However, building and reasoning over formal language have proved challenging (Musen and Van der Lei, 1988), with representative disadvantages of brittleness and knowledge-acquisition bottleneck. 

% Symbolic models identify the discrete symbols (like entities and logical functions) as basic reasoning units, and perform explicit inferences upon symbolic representations. With controllable and interpretable reasoning steps, yet they largely depend on expert-defined rules which are inflexible for different datasets and lack resilience against data noises [17]. 

% A typical symbolic AI system might consist of a knowledge base, which is typically hand-curated by
% experts, and an inference engine that allows the system to perform logic-based reasoning over its
% knowledge base. 

% One of the primary benefits of symbolic AI systems over deep learning models is their interpretability; we can look at the reasoning steps such a system has taken to see how the final conclusion was
% reached. However, unlike deep learning approaches, symbolic AI systems require knowledge to be
% hand-crafted and are in general hard to scale.


% LLMs often struggle with performing arithmetic operations [8, 9, 15]. To address this, [15] uses an external calculator to evaluate the arithmetic operations in the generated reasoning steps. Program-Aided Language model (PAL) [7] extends this idea by generating Python programs as reasoning steps, offloading all calculations to a Python interpreter. Although programs offer a direct representation of procedures

% To address the inherent limitations of LLMs, such as the inability to access up-to-date information, take actions, or perform precise mathematical reasoning, recent works have started to augment language models with access to external tools and resources. 

% Recently developed methods have shown that the performance of downstream tasks of LLMs can be improved by combining them with external modules. For instance, WebGPT [45] is a fine-tuned version of GPT-3 by combining web knowledge to answer open-ended questions. Lazaridou et al. studied how search engines like Google can be utilized as external tools for LLMs. MemPrompt [47] presented a human-in-the-loop system where a growing memory of errors and user feedback is served as past experience adding to the prompts for more accurately answering new questions. REPLUG [48] is another retrieval-augmented language modeling paradigm that treats the language model as a black box and augments it with a tuneable retrieval model. In very recent work related to ours, Schick et al. trained a model called ToolFormer that can decide when and how to call certain tool APIs by in-line augmentation on prompts for LLMs.In this work, we propose that classical planners can be another particularly useful external module.
% In comparison, LLM+P, does not rely on any fine-tuning or re-training of LLMs. By simply in- corporating knowledge from classical planners, LLM+P incorporates long-horizon reasoning and planning capabilities into existing LLMs.

% Some recent works aim to let the model access external knowledge that is not necessarily stored in their weights. For example, when it accesses a search engine to retrieve updated factual information. It may also have access to other tools such as calculators or code interpreters. In this line of research, we find different methods to retrieve information. For example, they may condition the LM on the retrieved documents \cite{atlas},  iterativeley query the search engine in their prompts  \cite{selfAsk}, \cite{demonstrate_search_predict}, \cite{finke98clarity}, \cite{react},  or get access to the web \cite{webgpt}. On the other side, we find another line of work that uses LLMs as a general interface to access pre-trained models for other tasks \cite{hugginggpt} \cite{generalPurposeInterface}. Finally, the ability to \textit{Plan+Act} has also been recently studied by researchers in the field of Embodied AI or robotics, where they aim to guide a virtual or a real robot with high-level commands in natural language. These commands need to be later divided into smaller tasks that can be executed by the robots \cite{innerMonologue} \cite{openWorldPlanning} \cite{languageToGoals}. The examples of LLMs creating a plan are not only limited to Embodied AI, we can also find examples where they are being used to generate code \cite{planningCodeGeneration}.

Problem Formulator

% To use Codex for our purposes, we take advantage of its few-shot generalization ability and we find that it can learn our defined grammar effectively with only a small number of in-context examples $\mathcal{D} = \{ d_1, \cdots, d_{|D|}\}$. Each example $d_i$ consists of the claim and the program. 

%  At inference time, we prompt Codex with an instruction of the task, K in-context examples, and the
% input claim C. Codex then attempts to complete
% the following texts, and thereby generate a program
% for C. The prompt template is shown in Figure 2.
% We use K = 20 in our experiments to maitain a
% tradeoff between the diversity of reasoning types
% and the model’s maximum input capacity.

% Few-shot prompting is a technique that uses LLMs to solve a task by providing the LLMs with a few demonstrations of the task as part of the input at inference time [1]. In this technique, the demonstrations (i.e., examples of input-output pairs) are concatenated into a prompt, which is passed to the model along with the new input to generate an output

% To solve a math word problem, we first use an LLM to formalize the problem as a set of variables and equations. Recently, using few-shot prompting over LLMs has emerged as an effective approach for natural language understanding and decomposition. 

% LLMs are bad at planning (or long-horizon reasoning) [9] but they are good at describing and translating textual inputs, including re-writing planning prompts in the PDDL format. The intuition is that we can view PDDL as a different language than English, so re-writing planning prompts in PDDL is essentially a “machine translation” task that LLMs are known to excel at. 

% LLMs are known to be capable of in-context learning without finetuning their parameters. By in- context learning, we mean LLMs’ ability to perform unseen downstream tasks by simply condition- ing on a few input-label pairs (demonstrations) [10]. Here is a pair of problem descriptions in natural language and in PDDL provided to GPT-4 as context. When the context is included with the prompt from the example above, the resulting PDDL problem file is directly solvable by the planner.



% Reasoning: 
% Reasoning with forward-chaining to derive additional facts. 
% Reasoning with backward-chaining to prove goals. 


% Logic programming is a symbolic system to describe deductive reasoning using facts and rules. 
% In this work, we adopt the key grammar of Prolog to formulate a problem into facts, rules, and queries. 
% Logic programming has long been used as a formal symbolic system to describe deductive reasoning, 
% Logic programming is a paradigm that uses a system of facts and rules. 

% What is deductive reasoning
% Logic programming has been long been used as a formal symbolic system to describe deductive reasoning, 
% Difference with Python, LP is a declarative language 
% describe rules, facts, and goals. Prolog~\cite{clocksin2003programming,DBLP:journals/tplp/KornerLBCDHMWDA22} is arguably the most prominent language under the logic programming (LP) umbrella.
% We follow the grammar of Prolog to 
% A deductive inference is to infer valid knowledge (conclusion) from the given knowledge (premises). 
% Logic programming is a paradigm that uses a system of facts and rules. It is commonly used in the artificial intelligence and machine learning domains. This guide explains the logic programming paradigm and compares it to other programming models. 
% Prolog is arguably the most prominent language under the logic programming (LP) umbrella. 

\begin{table}[!t]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{SR} & \multirow{2}{*}{Correct (\%)} & \multicolumn{2}{c}{Incorrect (\%)} \\ \cmidrule{4-5}
& & & Semantic & Syntax \\ \midrule
\multirow{2}{*}{ProntoQA} & $-$ &  & &  \\ 
& $+$ &  &  &  \\ \midrule
\multirow{2}{*}{ProofWriter} & $-$ &  & &  \\ 
& $+$ &  &  &  \\ \midrule
\multirow{2}{*}{FOLIO} & $-$ & 55.39 & 51.47 & 57.60 \\ 
& $+$ & 60.29~\up{4.9} & 12.74~\up{4.9} & 60.29~\up{4.9} \\ \midrule
\multirow{2}{*}{\tabincell{l}{Logical\\Deduction}} & $-$ &  & &  \\ 
& $+$ &  &  &  \\ \bottomrule
\end{tabular}%
}
\end{table}


\begin{table}[!t]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{SR} & Overall & \multicolumn{2}{c}{Executable} \\ \cmidrule{3-5}
& & Acc. & Rate (\%) & Acc. \\ \midrule
\multirow{2}{*}{ProntoQA} & $-$ &  & &  \\ 
& $+$ &  &  &  \\ \midrule
\multirow{2}{*}{ProofWriter} & $-$ &  & &  \\ 
& $+$ &  &  &  \\ \midrule
\multirow{2}{*}{FOLIO} & $-$ & 55.39 & &  \\ 
& $+$ & 60.29~\up{4.9} & 60.29~\up{4.9} & 60.29~\up{4.9} \\ \midrule
\multirow{2}{*}{\tabincell{l}{Logical\\Deduction}} & $-$ &  & &  \\ 
& $+$ &  &  &  \\ \bottomrule
\end{tabular}%
}
\end{table}
